An Experimental Urban Case Study with Various Data Sources and a Model for Traffic Estimation

Accurate estimation of the traffic state over a network is essential since it is the starting point for designing and implementing any traffic management strategy. Hence, traffic operators and users of a transportation network can make reliable decisions such as influence/change route or mode choice. However, the problem of traffic state estimation from various sensors within an urban environment is very complex for several different reasons, such as availability of sensors, different noise levels, different output quantities, sensor accuracy, heterogeneous data fusion, and many more. To provide a better understanding of this problem, we organized an experimental campaign with video measurement in an area within the urban network of Zurich, Switzerland. We focus on capturing the traffic state in terms of traffic flow and travel times by ensuring measurements from established thermal cameras by the city's authorities, processed video data, and the Google Distance Matrix. We assess the different data sources, and we propose a simple yet efficient Multiple Linear Regression (MLR) model to estimate travel times with fusion of various data sources. Comparative results with ground-truth data (derived from video measurements) show the efficiency and robustness of the proposed methodology.

==> name.tex <==
\begin{itemize}
    \item Haghani et.al (2010): Data Collection of Freeway Travel Time Ground Truth with Bluetooth Sensors
    \item The work evaluates bluethooth sensors as a potential ground-truth for travel time assessment.
    \item States the contribution in doing this different compared to other works that use vehicle probe data
    \item Results are compare to vehicle probe data. Nevertheless, the quality of Bluetooth sensor data heavily depends on the penetration in the system why the statement that the new sensors can be utilized as ground-truth data is questionable with a low sample-rate.
\end{itemize}

\begin{itemize}
    \item Yeon et al (2008): Travel time estimation on a freeway using Discrete Time Markov Chains
    \item Paper tackles the problem of travel time estimation models that tend to underestimate the travel time in congestion conditions
    \item Model implemented for freeway travel time estimation with Discrete Time Markov Chains
    \item Model shows deviation from the measured travel time with lower than 3\%
    \item Speed, volume, occupancy and travel time data were collected in a case study to validate the methodology and show the performance. 
\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
indirect, i.e., estimation :


\begin{itemize}
    \item Yildirimoglu and Geroliminis (2013): Experienced travel time prediction for congested freeways
    \item Travel time predictions based on loop detector data in California from which speed is calculated. 
    \item The authors developed a framework to predict travel times by including the following methodological pieces: a bottleneck identification algorithm, traffic regime clustering, a stochastic congestion maps for clustered data and an algorithm for a congestion search algorithm.
\end{itemize}


and a more practical approach ....

\begin{itemize}
    \item Shen et al. (2013): Practical approach for travel time estimation from point traffic detector data
    \item The work investigates travel time estimation
        from point traffic detector data. 
    \item The paper focuses on filling data gaps (spatiall and temporarly) by utilizing exponential moving average (EMA) to improve travel time estimates
    \item Additionally, the calculated speed estimates from detector data is transformed from Time-mean-speed (TMS) to Space-mean-speed (SMS) which also shows improvement in travel time estimates. The transformation is performed by fitting a linear regression.
    \item 
\end{itemize}

%%%
data fusion of LD with other data sources
%%%
\begin{itemize}
    \item Bhaskar et al. (2011): Fusing Loop Detector and Probe Vehicle Data to Estimate Travel Time Statistics on Signalized Urban Networks
    \item The work critices that a lot of research is producing average travel times whereas it could be the case that no vehicle expierences average travel times. 
    \item Extends the traditional travel time estimation with cumulative plots by taking into fusing the data with probe vehilce data.
    \item The methodology is validated with real-world data in Switzerland. 
\end{itemize}




%%%%
another measure - travel time reliability 
%%%

 \begin{itemize}
    \item Lyman et al (2008): Using Travel Time Reliability Measures to Improve Regional Transportation Planning and Operations
    \item Paper highlights the importance of Travel Time Realability (TTR)
    \item Concucts a literature review of different TTR definitions
    \item Analyses empirical data from Portland, Oregon and shows the dependency of time of the day and day of the week. 
\end{itemize}

\begin{itemize}
    \item Chen et al (2019): Data analytics approach for travel time reliability pattern analysis and prediction
    \item Work focuses on the Travel Time Realiability (TTR), which is an important measure to indicate the traffic states on freeways. 
    \item Study utilizes vehicle probe data to develop an Exponential Smoothing (ETS) models for the prediction TTR. 
    \item A case study is conducted on a road corridor with several different prediction results that show a reasonable MAPE (Mean Absolute Percentage Error).
    \item No comparison to an actually ground truth data-set; comparison is made to the vehicle probe data where the accurancy is a function that depends on the penetration rate.
\end{itemize}

%%
other other
%%

\begin{itemize}
    \item Sen et al. (1999): Variances of link travel time estimates: implications for optimal routes
    \item Investigate the effect of using travel times with high variance to calculate the minimum travel time. 
\end{itemize}



